Stability of Algebraic Neural Networks to Small Perturbations

Algebraic neural networks (AlgNNs) are composed of a cascade of layers each one associated to and algebraic signal model, and information is mapped between layers by means of a nonlinearity function. AlgNNs provide a generalization of neural network architectures where formal convolution operators are used, like for instance traditional neural networks (CNNs) and graph neural networks (GNNs). In this paper we study stability of AlgNNs on the framework of algebraic signal processing. We show how any architecture that uses a formal notion of convolution can be stable beyond particular choices of the shift operator, and this stability depends on the structure of subsets of the algebra involved in the model. We focus our attention on the case of algebras with a single generator.

==> figures/gnn_block_diagram_single_feature_uncolored.tex <==
% !TEX root = ../00_gnn_eusipco.tex

%\definecolor{my_blue}{rgb}{0, 0, 0.4}
\definecolor{my_blue}{rgb}{0.0314, 0.3569, 1.0000}

\def \myfactor {0.65}
\def \unit  {\myfactor cm}

% Definition of a block for block diagrams
\tikzstyle{block} = [ rectangle,
                      minimum width = \unit,
                      minimum height = \unit,
                      fill = blue!15,
                      draw = black,
                      text = black]

% Control the color and size of filter blocks                  
\tikzstyle{filter} = [block,
                      minimum width  = 3.0*\unit,
                      minimum height = 1.3*\unit,
                      fill=my_blue!50!cyan]

% Control the color and size of nonlinearity blocks 
\tikzstyle{nonlinearity} = [ filter,
                             minimum width  = 3.0*\unit,
                             fill = gray!30!white]
                             %fill = mygreen!15]

% Control separation between blocks
\def \deltainput     {( 0.0,-1.5)}
\def \deltaoutput    {( 0.0,-0.9)}
\def \deltalayer     {3.0}
\def \deltaconnector {0.95}
\def \deltasigma     {( 4, 0.0)}
\def \deltafeature   {1.5}

% The text that is displayed inside of filter blocks
\def \one   {$\displaystyle{\mathbf{y}_{1}  = \rho_{1}(a)\mathbf{x}}$}
\def \two   {$\displaystyle{\mathbf{y}_2  =  \rho_{2}(a)\mathbf{x}_{1}}$}
\def \three {$\displaystyle{\mathbf{y}_3  = \rho_{3}(a)\mathbf{x}_{2}}$}
% The text that is displayed inside of nonlinearity blocks
\def \sigmaone   {$\displaystyle{\mathbf{z}_{1} = {\eta_{1}} \Big[\, \mathbf{y}_1 \, \Big]}$}
\def \sigmatwo   {$\displaystyle{\mathbf{z}_{2} = {\eta_{2}} \Big[\, \mathbf{y}_2 \, \Big]}$}
\def \sigmathree {$\displaystyle{\mathbf{z}_{3} = {\eta_{3}} \Big[\, \mathbf{y}_3 \, \Big]}$}
\def \proyone   {$\displaystyle{\mathbf{x}_{1} = {P_{1}} \Big[\, \mathbf{z}_1 \, \Big]}$}
\def \proytwo   {$\displaystyle{\mathbf{x}_{2} = {P_{2}} \Big[\, \mathbf{z}_2 \, \Big]}$}
\def \proythree   {$\displaystyle{\mathbf{x}_{3} = {P_{3}} \Big[\, \mathbf{z}_3 \, \Big]}$}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BEGIN FIGURE CODE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
{\fontsize{7}{7}\selectfont\begin{tikzpicture}[scale = \myfactor]

  \pgfdeclarelayer{bg}     % declare background layer
  \pgfsetlayers{bg,main}   % set the order of the layers (main is the standard layer)

  % Draw input to GNN
  \node (input) [rectangle, minimum width = 0.1*\unit] {$\mathbf{x}$};
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Layer 1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Draw Layer 1 Filter block and Feature block
  \path (input)      ++ \deltainput node [filter]       (L1 Filter1) {\one};
  \path (L1 Filter1) ++ \deltasigma node [nonlinearity] (L1 F1)      {\sigmaone};
  \path (L1 F1) ++ \deltasigma node [nonlinearity] (L1 F2)      {\proyone};
  % Draw connectors for Layer 1
  %\path[draw, -stealth] (L1 Filter1.east) -- node [above] {$\mathbf{z}_1$} (L1 F1.west);
  \path[draw, -stealth] (L1 Filter1.east) -- node [above] {$\mathbf{y}_1$} (L1 F1.west);
  \path[draw, -stealth] (L1 F1.east) -- node [above] {$\mathbf{z}_1$} (L1 F2.west);

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Layer 2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Draw Layer 2 Filter block and Feature block
  \path (L1 Filter1) ++ (0,-\deltalayer) node [filter]       (L2 Filter1) {\two};
  \path (L2 Filter1) ++ \deltasigma      node [nonlinearity] (L2 F1)      {\sigmatwo};
  \path (L2 F1) ++ \deltasigma node [nonlinearity] (L2 F2)      {\proytwo};
  % Draw connectors for Layer 2
  \path[draw, -stealth] (L2 Filter1.east) --  node [above] {$\mathbf{y}_2$} (L2 F1.west);
  \path[draw, -stealth] (L2 F1.east) -- node [above] {$\mathbf{z}_2$} (L2 F2.west);  
  
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Layer 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Draw Layer 2 Filter block and Feature block
  \path (L2 Filter1) ++ (0,-\deltalayer) node [filter]       (L3 Filter1) {\three};
  \path (L3 Filter1) ++ \deltasigma      node [nonlinearity] (L3 F1)      {\sigmathree};
  \path (L3 F1) ++ \deltasigma node [nonlinearity] (L3 F2)      {\proythree};
  % Draw connectors for Layer 2
  %\path[draw, -stealth] (L3 Filter1.east) --  node [above] {$\mathbf{z}_3$} (L3 F1.west);
  \path[draw, -stealth] (L3 Filter1.east) --  node [above] {$\mathbf{y}_3$} (L3 F1.west);
  \path[draw, -stealth] (L3 F1.east) -- node [above] {$\mathbf{z}_3$} (L3 F2.west); 

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Connections across layers %%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % From input to layer 1
  \path[draw, -stealth] (input.south) -- (L1 Filter1.north);
  % From layer 1 to layer 2
  \path (L1 F2.south) ++ (0,-\deltaconnector) node [] (aux1) {};
  \path[draw, -stealth] (L1 F2.south) -- node [below right] {$\mathbf{x}_1$} (aux1.north) 
                                      --                         (aux1.north -| L2 Filter1.north) 
                                      -- node [above left]  {$\mathbf{x}_1$} (L2 Filter1.north);
  % From layer 2 to layer 3
  \path (L2 F2.south) ++ (0,-\deltaconnector) node [] (aux1) {};
  \path[draw, -stealth] (L2 F2.south) -- node [below right] {$\mathbf{x}_2$} (aux1.north) 
                                      --                         (aux1.north -| L2 Filter1.north) 
                                      -- node [above left]  {$\mathbf{x}_2$} (L3 Filter1.north);
  % From layer 3 to output
  \path[draw, -stealth] (L3 F2.south) -- ++ \deltaoutput -- ++ (0.3, 0) 
                        node [right]{$\mathbf{x}_3$};

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Light shades to signify layer groups   %%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{pgfonlayer}{bg} 
      % Shading for Layer 1  
      \path (L1 Filter1.west |- L1 F1.south) ++ (-0.3,-0.3)
           node [filter, anchor = south west,
                 fill = black!1, 
                 %minimum width  = 10.75*\unit,
                 minimum width  = 14*\unit,
                 minimum height = 1.9*\unit,] 
        (layer)
        {}; 
      %\path (layer.south east) ++ (0.0,0.0) node [above left] {\fontsize{6}{6}\selectfont Layer 1};
       \path (layer.south east) ++ (0.0,0.0) node [above left] {\fontsize{6}{6}\selectfont  $\mathbf{x}_{1}\in\mathcal{M}_{2}$};
 \path (layer.south east) ++ (0.0,1) node [above left] {\fontsize{6}{6}\selectfont  $a\in\mathcal{A}_{1}$};
  \path (layer.south east) ++ (0.0,0.5) node [above left] {\fontsize{6}{6}\selectfont  $\mathbf{y}_{1},\mathbf{z}_{1}\in\mathcal{M}_{1}$};
      % Shading for Layer 2  
      \path (L1 Filter1.west |- L2 F1.south) ++ (-0.3,-0.3)
           node [filter, anchor = south west,
                 fill = black!1, 
                 minimum width  = 14*\unit,
                 minimum height = 1.9*\unit,] 
        (layer)
        {}; 
      %\path (layer.south east) ++ (0.0,0.0) node [above left] {\fontsize{6}{6}\selectfont Layer 2};
      \path (layer.south east) ++ (0.0,0.0) node [above left] {\fontsize{6}{6}\selectfont  $\mathbf{x}_{2}\in\mathcal{M}_{3}$};
 \path (layer.south east) ++ (0.0,1) node [above left] {\fontsize{6}{6}\selectfont  $a\in\mathcal{A}_{2}$};
  \path (layer.south east) ++ (0.0,0.5) node [above left] {\fontsize{6}{6}\selectfont  $\mathbf{y}_{2},\mathbf{z}_{2}\in\mathcal{M}_{2}$};
      % Shading for Layer 3  
      \path (L1 Filter1.west |- L3 F1.south) ++ (-0.3,-0.3)
           node [filter, anchor = south west,
                 fill = black!1, 
                 minimum width  = 14*\unit,
                 minimum height = 1.9*\unit,] 
        (layer)
        {}; 
      \path (layer.south east) ++ (0.0,0.0) node [above left] {\fontsize{6}{6}\selectfont  $\mathbf{x}_{3}\in\mathcal{M}_{\text{out}}$};
 \path (layer.south east) ++ (0.0,1) node [above left] {\fontsize{6}{6}\selectfont  $a\in\mathcal{A}_{3}$};
  \path (layer.south east) ++ (0.0,0.5) node [above left] {\fontsize{6}{6}\selectfont  $\mathbf{y}_{3},\mathbf{z}_{3}\in\mathcal{M}_{3}$};
  \end{pgfonlayer}

\end{tikzpicture}} 


==> sec_SpectOP.tex <==
%!TEX root = journal_AlgNN_v08.tex

\section{Spectral Operators}\label{sec:spectopt}
Before we proof the theorems presented in previous section, it is important to discuss the concept of \textit{Fourier decomposition} in the context of representation theory of algebras. We want to highlight specially the role of the filters when a representation is compared to its perturbed version. In particular, we will show that there are essentially two factors that can cause  differences between operators and their perturbed versions, the eigenvalues\footnote{As we will show later, this is indeed a particular case of a general notion of homomorphism between the algebra and an irreducible subrepresentation of $\mathcal{A}$.} and eigenvectors. Additionally, we show how the algebra can only affect one of those sources. This is consistent with the fact that differences in the eigenvectors of the operators only affect the constants that are associated to the stability bounds.

We highlight that the concept of spectral decomposition exploited extensively in traditional signal processing can be considered as a particular case of the concept of direct sums\footnote{When considering representations of non-compact groups this concept is insufficient and it is replaced for the more general notion of \textit{direct integral of Hilbert spaces}~\cite{folland2016course,deitmar2014principles}} of \textit{irreducible} representations. In this section we provide some basic definitions from the representation theory of algebras and its connection with the notion of spectral decomposition of signals in algebraic neural networks.  This will be useful and necessary in Section~\ref{sec:proofofTheorems} as the norm of the operators considered can be calculated in the terms of an spectral representation. We start with the following definition.
%%
%%------------------------Subsection---------------------------------
%\subsection{Finite and Countable infinite Dimensional Representations}
\begin{definition}
Let $(\mathcal{M},\rho)$ be a representation of $\mathcal{A}$. Then, a representation $(\mathcal{U},\rho)$ of $\mathcal{A}$ is a \textbf{subrepresentation} of  $(\mathcal{M},\rho)$ if $\mathcal{U}\subseteq\mathcal{M}$ and $\mathcal{U}$ is invariant under all operators $\rho(a)~\forall~a\in\mathcal{A}$, i.e. $\rho(a)u\in\mathcal{U}$ for all $u\in\mathcal{U}$ and $a\in\mathcal{A}$. A representation $(\mathcal{M}\neq 0,\rho)$ is \textbf{irreducible} or simple if the only subrepresentations of $(\mathcal{M}\neq 0,\rho)$ are $(0,\rho)$ and $(\mathcal{M},\rho)$.
\end{definition}
%
The class of irreducible representations of an algebra $\mathcal{A}$ is denoted by $\text{Irr}\{\mathcal{A}\}$. Notice that the zero vector space and $\mathcal{M}$ induce themselves subrepresentations of $(\mathcal{M},\rho)$. In order to state a comparison between representations the concept of \textit{homomorphism between representations} is introduced in the following definition.
%%
%%------------------------ Definition -----------------------------------------
\begin{definition}\label{def:homrep}
Let $(\mathcal{M}_{1},\rho_{1})$ and $(\mathcal{M}_{2},\rho_{2})$ be two representations of an algebra $\mathcal{A}$. A homomorphism or \textbf{interwining operator} $\phi:\mathcal{M}_{1}\rightarrow\mathcal{M}_{2}$ is a linear operator which commutes with the action of $\mathcal{A}$, i.e.
\begin{equation}
\phi(\rho_{1}(a)v)=\rho_{2}(a)\phi(v).
\label{eq:interwinop}
\end{equation}
A homomorphism $\phi$ is said to be an isomorphism of representations if it is an isomorphism of vectors spaces. 
\end{definition}
%%
%%
Notice from definition~\ref{def:homrep}  a substantial difference between the concepts of isomorphism of vector spaces and  isomorphism of representations. In the first case we can consider that two arbitray vector spaces of the same dimension (finite) are isomorphic, while for representations that condition is required but still the condition in eqn.~(\ref{eq:interwinop}) must be satisfied. For instance, as pointed out in~\cite{repthysmbook} all the irreducible 1-dimensional representations of the polynomial algebra $\mathbb{C}[t]$ are non isomorphic.

As we have discussed before, the vector space $\mathcal{M}$ associated to $(\mathcal{M},\rho)$  provides the space where the signals are modeled. Therefore, it is of central interest to determine whether it is possible or not to \textit{decompose} $\mathcal{M}$ in terms of simpler or smaller spaces consistent with the action of $\rho$.  We remark that for any two representations $(\mathcal{M}_{1},\rho_{1})$ and $(\mathcal{M}_{2},\rho_{2})$ of an algebra $\mathcal{A}$, their direct sum is given by the representation $(\mathcal{M}_{1}\oplus\mathcal{M}_{2},\rho)$ where $\rho(a)(\mathbf{x}_{1}\oplus\mathbf{x}_{2})=(\rho_{1}(a)\mathbf{x}_{1}\oplus\rho_{2}(a)\mathbf{x}_{2})$. We introduce the concept of indecomposability in the following definition.
%%
%%------------------------ Definition ------------------------------------------
\begin{definition}\label{def:indecomprep}
A nonzero representation $(\mathcal{M},\rho)$ of an algebra $\mathcal{A}$ is said to be \textbf{indecomposable} if it is not isomorphic to a direct sum of two nonzero representations.
\end{definition}
%%
%%
Indecomposable representations provide the \textit{minimum units of information} that can be extracted from signals in a given space when the filters have a specific structure (defined by the algebra)~\cite{barot2014introduction}. The following theorem provides the basic building block for the decomposition of finite dimensional representations.
%%
%%-----------------------------Theorem-------------------------------------------
\begin{theorem}[Krull-Schmit, \cite{repthybigbook}]\label{theorem:krullschmitdecomp}
Any finite dimensional representation of an algebra can be decomposed into a finite direct sum of indecomposable subrepresentations and this decomposition is unique up to the order of the summands and up to isomorphism. 
\end{theorem}
%%
%%
The uniqueness in this result means that if $(\oplus_{r=1}^{r}V_{i},\rho)\cong(\oplus_{j=1}^{s}W_{j},\gamma)$ for indecomposable representations $(V_{j},\rho_{j}),(W_{j},\gamma_{j})$, then $r=s$ and there is a permutation $\pi$ of the indices such that $(V_{i},\rho_{i})\cong (W_{\pi(j)},\gamma_{\pi(j)})$~\cite{repthybigbook}. Although theorem~\ref{theorem:krullschmitdecomp} provides the guarantees for the decomposition of representation in terms of indecomposable representations, it is not applicable when infinite dimensional representations are considered. However, it is possible to overcome this obstacle taking into account that irreducible representations are indecomposable~\cite{repthysmbook,repthybigbook}, and they can be used then to build representations that are indecomposable. In particular, \textit{irreducibility} plays a central role to decompose the invariance properties of the images of $\rho$ on $\text{End}(\mathcal{M})$~\cite{repthybigbook}. Representations that allow a decomposition in terms of subrepresentations that are irreducible are called \textit{completely reducible} and its formal description is presented in the following definition.
%%
%%-----------------------------Definition-----------------------------------------
\begin{definition}[~\cite{repthybigbook}]\label{def:complredu}
 A representation $(\mathcal{M},\rho)$ of the algebra $\mathcal{A}$ is said to be \textbf{completely reducible} if $(\mathcal{M},\rho)=\bigoplus_{i\in I}(\mathcal{U}_{i},\rho_{i})$ with irreducible subrepresentations $(\mathcal{U}_{i},\rho_{i})$. The \textbf{length} of $(\mathcal{M},\rho)$ is given by $\vert I\vert$.
\end{definition}
%%
%%
%Irreducible representations are indecomposable, therefore by using irreducible representations it is possible to decompose an arbitrary representation where the minimum component in the decomposition has an \textit{invariance property}.  

For a given $(\mathcal{U},\rho_{\mathcal{U}})\in\text{Irr}\{\mathcal{A}\}$ the sum of all irreducible subrepresentations of $(V,\rho_{V})$ that are equivalent (isomorphic) to $(\mathcal{U},\rho_{\mathcal{U}})$ is represented by $V(\mathcal{U})$ and it is called the $\mathcal{U}$-homogeneous component of $(V,\rho_{V})$. This sum is a direct sum, therefore it has a length that is well defined and whose value is called the \textit{multiplicity} of $(\mathcal{U},\rho_{\mathcal{U}})$ and is represented by $m(\mathcal{U},V)$~\cite{repthybigbook}. Additionally, the sum of all irreducible subrepresentations of $(V,\rho_{V})$ will be denoted as $\text{soc}\{V\}$. It is possible to see that a given representation $(V,\rho_{V})$ is completely reducible if and only if $(V,\rho_{V})=\text{soc}\{S\}$~\cite{repthybigbook}. The connection between $\text{soc}\{V\}$ and $V(\mathcal{U})$ is given by the following proposition. 
%%
%%---------------------------Proposition-------------------------------------
\begin{proposition}[Proposition 1.31~\cite{repthybigbook}]\label{prop:repdirectsum1}
Let $(V,\rho_{V})\in\mathsf{Rep}\{A\}$. Then $\text{soc}\{V\}=\bigoplus_{S\in\text{Irr}\{\mathcal{A}\}}V(S)$.
\end{proposition}
%%
%%
Now, taking into account that any homogeneous component $V(\mathcal{U})$ is itself a direct sum we have that 
\begin{equation}
\text{soc}\{V\}\cong\bigoplus_{S\in\text{Irr}\{\mathcal{A}\}}S^{\oplus m(\mathcal{U},V)}.
\label{eq:repdirectsumtot}
\end{equation}
Equation~(\ref{eq:repdirectsumtot}) provides the building block for the definition of Fourier decompositions in algebraic signal processing~\cite{algSP1}. With all these concepts at hand we are ready to introduce the following definition.
%%
%%-----------------------------Definition------------------------------------------
\begin{definition}[Fourier Decomposition]\label{def:foudecomp}
For an algebraic signal model $(\mathcal{A},\mathcal{M},\rho)$ we say that there is a spectral or Fourier decomposition of $(\mathcal{M},\rho)$ if
\begin{equation}
(\mathcal{M},\rho)\cong\bigoplus_{(\mathcal{U}_{i},\phi_{i})\in\text{Irr}\{\mathcal{A}\}}(\mathcal{U}_{i},\phi_{i})^{\oplus m(\mathcal{U}_{i},\mathcal{M})}
 \label{eq:foudecomp1}
\end{equation}
where the $(\mathcal{U}_{i},\phi_{i})$ are irreducible subrepresentations of $(\mathcal{M},\rho)$. Any signal $\mathbf{x}\in\mathcal{M}$ can be therefore represented by the map $\Delta$ given by 
\begin{equation}
\begin{matrix} 
\Delta: & \mathcal{M} \to \bigoplus_{(\mathcal{U}_{i},\phi_{i})\in\text{Irr}\{\mathcal{A}\}}(\mathcal{U}_{i},\phi_{i})^{\oplus m(\mathcal{U}_{i},\mathcal{M})} \\ & \mathbf{x}\mapsto \hat{\mathbf{x}}
 \end{matrix}
 \label{eq:foudecomp2}
\end{equation}
known as the Fourier decomposition of $\mathbf{x}$ and the projection of $\hat{\mathbf{x}}$ in each $\mathcal{U}_{i}$ are the Fourier components represented by $\hat{\mathbf{x}}(i)$.
\end{definition}
%%
%%
%\begin{figure}
% \centering\includegraphics[scale=1,angle=0]{../figures/fig9.pdf}
%  \caption{Diagram indicating the maps and the spaces when a completely reducible representation $(\mathcal{M},\rho)$ is decomposed as a direct sum of irreducible subrepresentations.}
%  \label{fig_3}
%\end{figure}
%%
%%
Notice that in eqn.~(\ref{eq:foudecomp1}) there are two sums, one dedicated to the non isomorphic subrepresentations (external) and another one (internal) dedicated to subrepresentations that are isomorphic. In this context, the sum for non isomorphic representations indicates the sum on the \textit{frequencies} of the representation while the sum for isomorphic representations a sum of components associated to a given frequency. It is also worth pointing out that $\Delta$ is an interwining operator, therefore, we have that $\Delta(\rho(a)\mathbf{x})=\rho(a)\Delta(\mathbf{x})$. As pointed out in~\cite{algSP0} this can be used to define a convolution operator as $\rho(a)\mathbf{x}=\Delta^{-1}(\rho(a)\Delta(\mathbf{x}))$. The projection of a filtered signal $\rho(a)\mathbf{x}$ on each $\mathcal{U}_{i}$ is given by $\phi_{i}(a)\hat{\mathbf{x}}(i)$ and the collection of all this projections is known as the \textit{spectral representation} of the operator $\rho(a)$. Notice that $\phi_{i}(a)\hat{\mathbf{x}}(i)$ translates to different operations depending on the dimension of $\mathcal{U}_{i}$. For instance, if $\text{dim}(\mathcal{U}_{i})=1$, $\hat{\mathbf{x}}(i)$ and $\phi_{i}(a)$ are scalars while if $\text{dim}(\mathcal{U}_{i})>1$ and finite $\phi_{i}(a)\hat{\mathbf{x}}(i)$ is obtained as a matrix product.
%
%
%In many important applications the $\mathcal{U}_{i}$ in eqn.~(\ref{eq:foudecomp1}) are one dimensional spaces~\cite{algSP0,algSP1,algSP3}, that when seen as homogeneous components of a representation $(V,\rho_{V})$  became of particular interest as they are connected with the traditional concepts of eigenspaces and eigenvalues~\cite{repthybigbook}. Indeed, eigenspaces can be considered particular cases of the so called \textit{weight spaces}, introduced in the following definition.
%%%
%%%---------------------------Definition-----------------------------------------
%\begin{definition}[Weight spaces~\cite{repthybigbook}]\label{def:weightspaces}
%Let $(\mathcal{U},\phi)$ be a 1-dimensional representation of an algebra $\mathcal{A}$. Then the $\mathcal{U}-$homogeneous component $V(\mathcal{U})$ is given by
%\begin{equation}
%V(\mathcal{U})=\left\lbrace v\in V\vert \rho(a)v=\phi(a)v~\forall~a\in\mathcal{A}\right\rbrace 
%\label{eq:weightspaces}
%\end{equation}
%if $V(\mathcal{U})\neq 0$, then $\phi$ is called a \textbf{weight} of the representation $(V,\rho_{V})$ and $V(\mathcal{U})$ is called the corresponding \textbf{weight space}.
%\end{definition}
%%%
%%%
%In the context of definition~\ref{def:weightspaces} it is important to point out that when $\mathcal{A}=\mathbb{K}[t]$ and  $\phi(t)=\lambda\in\mathbb{K}$, $V(\mathcal{U})$ is the usual eigenspace for the eigenvalue $\lambda$ of the endomorphism $\rho(t)$. However when the algebra is not polynomial eqn.(~\ref{eq:weightspaces}) offers a generalization that allows to define more general spectral representations. 

%When considering definition~(\ref{def:foudecomp}) and eqn.(\ref{eq:foudecomp2}) with one dimensional subrepresentations the spectral representation of the operator $\rho(a)$ is given by
%\begin{equation}
%\rho(a)\mathbf{x}=\sum_{i}\hat{\mathbf{x}}(i)\phi_{i}(a)\mathbf{u}_{i}
%\label{eq:spectopt}
%\end{equation}
%where $\mathbf{u}_{i}$ is the basis vector associated to $\mathcal{U}_{i}$.
%%
%%-------------------------Remark--------------------------------------------------------------
\begin{remark}\label{remark:interpSpecFilt}\normalfont
The spectral representation of an operator indicated as $\phi_{i}(a)\hat{\mathbf{x}}(i)$ and eqns.~(\ref{eq:foudecomp1}) and~(\ref{eq:foudecomp2}) highlight one important fact that is essential for the discussion of the results in Section~\ref{sec:proofofTheorems}. For a completely reducible representation $(\mathcal{M},\rho)\in\mathsf{Rep}\{\mathcal{A}\}$ the connection between the algebra $\mathcal{A}$ and the spectral representation is \textit{exclusively} given by $\phi_{i}(a)$ which is acting on $\hat{\mathbf{x}}(i)$, therefore, it is not possible by the selection of elements or subsets of the algebra to do any modification on the spaces $\mathcal{U}_{i}$ associated to the irreducible components in eqn.(\ref{eq:foudecomp1}). As a consequence, when measuring the similarities between two operators $\rho(a)$ and $\tilde{\rho}(a)$ associated to $(\mathcal{M},\rho)$ and $(\mathcal{M},\tilde{\rho})$, respectively, there will be two sources of error. One source of error that can be modified by the selection of $a\in\mathcal{A}$ and another one that will be associated with the differences between spaces $\mathcal{U}_{i}$ and $\tilde{\mathcal{U}}_{i}$, which are associated to the direct sum decomposition of $(\mathcal{M},\rho)$ and $(\mathcal{M},\tilde{\rho})$, respectively. This point was first elucidated in~\cite{fern2019stability} for the particular case of GNNs, but it is part of a much more general statement that becomes more clear in the language of algebraic signal processing. 
\end{remark}
%%
%%
%%------------------------------Subsection----------------------------
%%
%\subsection{Examples}
%%
%\subsubsection{CNNs}
\begin{example}[Discrete signal processing]\normalfont
In CNNs the filtering is defined by the polynomial algebra $\mathcal{A}=\mathbb{C}[t]/(t^{N}-1)$, therefore, in a given layer the spectral representation of the filters is given by
%
\begin{multline*}
\rho(a)\mathbf{x}=\sum_{i=1}^{N}\phi_{i}\left(\sum_{k=0}^{K-1}h_{k}t^{k}\right)\hat{\mathbf{x}}(i)\mathbf{u}_{i}\\
=\sum_{i=1}^{N}\sum_{k=0}^{K-1}h_{k}\phi_{i}(t)^{k}\hat{\mathbf{x}}(i)\mathbf{u}_{i}
=\sum_{i=1}^{N}\sum_{k=0}^{K-1}h_{k}\left(e^{-\frac{2\pi ij}{N}}\right)^{k}\hat{\mathbf{x}}(i)\mathbf{u}_{i},
\end{multline*}
%
with $a=\sum_{k=0}^{K-1}h_{k}t^{k}$ and where the $\mathbf{u}_{i}(v)=\frac{1}{\sqrt{N}}e^{\frac{2\pi jvi}{N}}$ are the column vectors of the traditional DFT matrix, while $\phi_{i}(t)=e^{-\frac{2\pi ji}{N}}$ is the eigenvalue associated to $\mathbf{u}_{i}$. Here $\hat{\mathbf{x}}$ represents the DFT of $\mathbf{x}$.
\end{example}
%%
%%---------------------------------Subsection-----------------------------------
\begin{example}[Graph signal processing]\normalfont
Taking into account that the filtering in each layer of a GNN is defined by a polynomial algebra, the spectral representation of the filter is given by
%
\begin{multline}
\rho(a)\mathbf{x}=\sum_{i=1}^{N}\phi_{i}\left(\sum_{k=0}^{K-1}h_{k}t^{k}\right)\hat{\mathbf{x}}(i)\mathbf{u}_{i}\\
=\sum_{i=1}^{N}\sum_{k=0}^{K-1}h_{k}\phi_{i}(t)^{k}\hat{\mathbf{x}}(i)\mathbf{u}_{i}=
\sum_{i=1}^{N}\sum_{k=0}^{K-1}h_{k}\lambda_{i}^{k}\hat{\mathbf{x}}(i)\mathbf{u}_{i}
\label{eq:specopgnn}
\end{multline}
%
with $a=\sum_{k=0}^{K-1}h_{k}t^{k}$, and where the $\mathbf{u}_{i}$ are given by the eigenvector decomposition of $\rho(t)=\mathbf{S}$, where $\mathbf{S}$ could be the adjacency matrix or the Laplacian of the graph, while $\phi_{i}(t)=\lambda_{i}$ being $\lambda_{i}$ the eigenvalue associated to $\mathbf{u}_{i}$. The projection of $\mathbf{x}$ in each subspace $\mathcal{U}_{i}$ is given by $\hat{\mathbf{x}}(i)=\langle\mathbf{u}_{i}, \mathbf{x}\rangle$, and if $\mathbf{U}$ is the matrix of eigenvectors of $\mathbf{S}$ we have the widely known representation $\hat{\mathbf{x}}=\mathbf{U}^{T}\mathbf{x}$~\cite{gamagnns}.
\end{example}
%%
%%-------------------Example--------------------------------
\begin{example}[Group signal processing]\label{example:specopGroupCNNs}
\normalfont
Considering the Fourier decomposition on  general groups~\cite{steinbergrepg,terrasFG,fulton1991representation}, we obtain the spectral representation of the algebraic filters as
\begin{equation*}
\boldsymbol{a}\ast\mathbf{x}=\sum_{u,h\in G}\boldsymbol{a}(uh^{-1})\sum_{i,j,k}\frac{d_{k}}{\vert G\vert}\hat{\mathbf{x}}\left(\boldsymbol{\varphi}^{(k)}\right)_{i,j}\boldsymbol{\varphi}_{i,j}^{(k)}(h)hu,
\end{equation*}
where $\hat{\mathbf{x}}(\boldsymbol{\varphi}^{(k)})$ represents the Fourier components associated to the $k$th irreducible representation with dimension $d_{k}$ and $\boldsymbol{\varphi}^{(k)}$ is the associated unitary element. We can see that the $k$th element in this decomposition is $\sum_{i,j}\mathbf{x}(\varphi^{(k)})_{i,j}\sum_{u,h}\frac{d_{k}}{\vert G\vert}\boldsymbol{a}(uh^{-1})\boldsymbol{\varphi}_{i,j}^{(k)}(h)hu$.
\end{example}
%%
%%-------------------Subsection--------------------------------
%\subsubsection{CNNs, with infinite dimensional representations}
\begin{example}[Graphon signal processing]\normalfont
According to the spectral theorem~\cite{conway1994course,aliprantis2002invitation}, it is possible to represent the action of a compact normal operator $S$ as $S\mathbf{x}=\sum_{i}\lambda_{i}\langle\boldsymbol{\varphi}_{i},\mathbf{x}\rangle\boldsymbol{\varphi}_{i}$ where $\lambda_{i}$ and $\boldsymbol{\varphi}_{i}$ are the eigenvalues and eigenvectors of $S$, respectively, and $\langle\cdot\rangle$ indicates an inner product. Then, the spectral representation of the filtering of a signal in the layer $\ell$ is given by
\begin{equation*}
\rho_{\ell}\left(p(t)\right)\mathbf{x}
=
\sum_{i}p(\lambda_{i})\langle\mathbf{x},\boldsymbol{\varphi}_{i}\rangle\boldsymbol{\varphi}_{i}=\sum_{i}\phi_{i}(p(t))\hat{\mathbf{x}}_{i}\boldsymbol{\varphi}_{i},
\end{equation*}
where $\phi_{i}(p(t))=p(\lambda_{i})$.
\end{example}










==> sec_algNN.tex <==

%%---------------------------------------------------------------------
%%---------SECTION: ALGEBRAIC NEURAL NETWORKS -------------------------
%%---------------------------------------------------------------------



\section{Algebraic Neural Networks}
\subsection{Convolution Feaures}
\subsection{Pooling}

==> sec_discussion.tex <==
%%--------------------------------------------------------------------
%%---------------- SECTION: DISCUSSION--------------------------------
%%--------------------------------------------------------------------
%
\section{Discussion}\label{sec:discussion}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t]
    \centering
    \input{./source_figs/plots_stability/graph_dilation_unstable.tex}\medskip
    \input{./source_figs/plots_stability/graph_dilation_stable.tex}    
   \caption{Filter properties and stability for algebraic operators considering algebras with a single generator. (Top) We depict a Lipschitz filter where it is possible to see that an arbitrary degree of selectivity can be achieved in any part of the spectrum. (bottom) We depict a Lipschitz integral filter where we can see how the magnitude of the filters tends to a constant value as the size of $\vert\lambda_{i}\vert$ grows. As a consequence there is no discriminability in one portion of the spectrum.}
 \label{fig_graph_dilation}
\end{figure}
%
%\medskip \noindent {\bf Perturbation analysis and selectivity in spectrum} 
The mathematical form of the notion of stability introduced in definition~(\ref{def:stabilityoperators1}), eqn.~(\ref{eq:stabilityoperators1}) is uncannily similar to the expressions associated to the stability conditions stated in~\cite{mallat_ginvscatt,bruna_iscn} when the perturbation operator $\tau$  considered was affecting directly the domain of the signals.  This is consistent with the fact that  the size of the perturbation on the operators is the size of an induced diffeomorphism $\mathbf{T}$ acting on $\text{End}(\mathcal{M})$. Measuring the size of perturbations in this way, although less intuitive, provides an alternative way to handle and interpret perturbations on irregular domains. 

The nature and severity of the perturbations, imposes restrictions on the behavior of the filters needed to guarantee stability. The more complex and severe the perturbation is the more conditions  on the filters are necessary to guarantee stability. This in particular has implications regarding to the selectivity of the filters in some specific frequency bands. The trade-off between stability and selectivity in the filters of the AlgNN can be measured by the size of the upper bounds in Theorems~\ref{theorem:HvsFrechet} up to~\ref{theorem:stabilityAlgNN1}, in particular, the size of $L_{0}$ and $L_{1}$ associated to the boundedness of the derivatives of the elements in $\mathcal{A}_{L0}$ and $\mathcal{A}_{L1}$. The smaller the value of $L_{0}, L_{1}$ the more stable the operators but the less selectivity we have. In Fig.~(\ref{fig_graph_dilation}) the properties in frequency of Lipschtiz and Lipschitz integral filters are depicted, where it is possible to see how the selectivity on portions of the spectrum is affected by properties that at the same time provide stability conditions for the perturbation models considered. 

It is important to remark that the function $\sigma_{\ell}=P_{\ell}\circ\eta_{\ell}$ composed by the projection operator $P_{\ell}$ and the nonlinearity function $\eta_{\ell}$ relocates information from one layer to the other performing a mapping between different portions of the spectrum associated to each of the spaces $\mathcal{M}_{\ell}$.  As $\eta_{\ell}$ maps elements of $\mathcal{M}_{\ell}$ onto itself,  we can see in light of the decomposition of $\mathcal{M}_{\ell}$ in terms of irreducible representations that 
$\eta_{\ell}$ is nothing but a relocator of information from one portion of the spectrum to the other. Additionally, the simplicity of $\eta_{\ell}$ provides  a rich variety of choices that can be explored in future research. 

The notion of differentiability between metric spaces or Banach spaces can be considered also using the notion of \textit{G\^ateaux derivative} which is considered a \text{weak} notion of differentiability. Although Gateaux differentiability is in general different from Fr\'echet  differentiability, it is possible to show that when $\text{dim}\left(\text{End}(\mathcal{M})\right)<\infty$ both notions are equivalent for Lipschtiz functions, but substantial differences may exist if $\text{dim}\left(\text{End}(\mathcal{M})\right)=\infty$ even if the functions are Lipschitz~\cite{benyamini2000geometric,lindenstrauss2012frechet}. 








==> sec_multiplegenresults.tex <==
\green{

\section{Multiple Generators}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% THEOREM %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{theorem}\label{theorem:uppboundDHmultg}
Let $\mathcal{A}$ be an algebra with $m$ generators $\{g_{i}\}_{i=1}^{m}$ and $g_{i}g_{j}=g_{j}g_{i}$ for all $i,j\in\{1,\ldots m\}$. Let $(\mathcal{M},\rho)$ be a finite or countable infinite dimensional representation of $\mathcal{A}$ and $(\mathcal{M},\tilde{\rho})$ a perturbed version of $(\mathcal{M},\rho)$ related by the perturbation model in eqn.~(\ref{eq:perturbmod1}).  Then, if $p_{\mathcal{A}}\in\mathcal{A}_{L_{0}}\cap\mathcal{A}_{L_{1}}$ it holds that
%
\begin{multline}
\left\Vert D_{p_{\mathcal{M}}\vert\mathbf{S}_{i}}(\mathbf{S})\bbT(\bbS_{i})\right\Vert\leq
\\
(1+\delta_{0})L_{0}\sup_{\bbS_{i}\in\mathcal{S}}\Vert\bbT(\bbS_{i})\Vert +\left(1+q\delta\right)E_{q}L_{1}\sup_{\bbS_{i}\in\mathcal{S}}\Vert D_{\bbT}(\bbS_{i})\Vert
\label{eq:DHTSmultg}
\end{multline}
 \end{theorem}





--- CALCULATING the Frechet Derivative-------
\begin{proof}
$p(\mathbf{S})=p(\mathbf{S}_{1},\mathbf{S}_{2},\ldots,\mathbf{S}_{m})$, then

\begin{multline}
p(\mathbf{S}+\boldsymbol{\xi})-p(\mathbf{S})
\\
=\sum_{k_{1},\ldots,k_{m}=0}^{\infty}h_{k_{1},\ldots k_{m}}(\mathbf{S}_{1}+\boldsymbol{\xi}_{1})^{k_{1}}(\mathbf{S}_{2}+\boldsymbol{\xi}_{2})^{k_{2}}\cdots (\mathbf{S}_{m}+\boldsymbol{\xi}_{m})^{k_{m}}
\\
-\sum_{k_{1},\ldots,k_{m}=0}^{\infty}h_{k_{1},\ldots k_{m}}\mathbf{S}_{1}^{k_{1}}\mathbf{S}_{2}^{k_{2}}\ldots\mathbf{S}_{m}^{k_{m}}
\\
=D_{p\vert\mathbf{S}_{1}}(\mathbf{S})+\ldots +D_{p\vert\mathbf{S}_{m}}(\mathbf{S})+N(\boldsymbol{\xi})
\end{multline}
%
%
\end{proof}
}

==> sec_quivrep.tex <==
%!TEX root = quiverSP_v00.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% INTRODUCTION %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Quiver Representations}
\label{sec:quivrep}



%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% FIGURE  %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{figure}
%	\centering
%\includegraphics[width=0.2\textwidth]{../figs/fig1.pdf}
%\includegraphics[width=0.2\textwidth]{../figs/fig2.pdf}
%\caption{A quiver $Q$ (left) and one  particular representation (right) of $Q$. $\mathcal{V}_{i}$ is a vector space associated to the node $i$ of the quiver while $\phi_{i,j}$ is a linear map between the spaces $\mathcal{V}_{i}$ and $\mathcal{V}_{j}$.}
%\label{fig:quiver1}
%\end{figure}


Informally speaking a quiver is a directed graph where multiple edges and loops are allowed, but in order to facilitate the introduction of the concept of representation we require a more formal definition that we introduce next. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% DEFINITION %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{definition}\label{def:quiver}
A quiver $Q$ is a quadruple $Q=(Q_{0},Q_{1},h,t)$ wehre $Q_{0}$ is a finite set of vertices, $Q_{1}$ is a finite set of arrows, and $h$ and $t$ are functions $Q_{1}\rightarrow Q_{0}$. For an arrow $a\in Q_{1}$, h(a) and $t(a)$ are called the head and the tail of $a$.
\end{definition}



%%
%%---------------------------------------Example---------------------------------------------------------------------
%%
\begin{example}\label{example:1}\normalfont
Let us consider the quiver indicated in Fig.~\ref{fig:quiver1} composed by the nodes $Q_{0}=\{1,2,3,4,5\}$ and the arrows $Q_{1}=\{a_{1,2}, a_{2,3},a_{2,2},a_{3,4},a_{3,5},a_{4,4},a_{4,1},a_{5,1}\}$. In this case we have that the functions $h$ and $t$ are given by $h(a_{i,j})=j$ and $t(a_{i,j})=i$.
\end{example}

Notice that the quiver itself does not offer anything new that has not been considered in the GSP literature. No structure is provided or associated to the graph. However, the notion of representation of a quiver provides the basic and formal components that can be used to associate information to the quiver in different ways. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%----------------------------------- DEFINITION -----------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{definition}
A representation $\boldsymbol{\pi}$ of a quiver $Q=(Q_{0},Q_{1},h,t)$ consists of a collection of vector spaces $\mathcal{V}_{i}$ associated to the \textbf{nodes} $i$, i.e. $\boldsymbol{\pi}(i)=\mathcal{V}_{i}$ for $i\in Q_{0}$ and a set of linear maps $\phi_{i,j}$ associated to the arrows, $\phi_{i,j}=\boldsymbol{\pi}(a_{i,j})$. Additionally, a representation $\boldsymbol{\theta}$ is called a subrepresentation of a representation $\boldsymbol{\pi}$ if $\boldsymbol{\theta}(x)$ is a subspace $\boldsymbol{\pi}(x)$ for all $x\in Q_{0}$, and $\boldsymbol{\pi}(a):\boldsymbol{\pi}(t(a))\rightarrow\boldsymbol{\pi}(h(a))$ restricts to $\boldsymbol{\theta}(a):\boldsymbol{\theta}(t(a))\rightarrow\boldsymbol{\theta}(h(a))$ for all $a\in Q_{1}$.
\end{definition}
%
%%------------------------------ End of DEFINITION -----------------------------------------------------------------

To show the versatility of a quiver representation to endow a directed graph with structure we recall the example~\ref{example:1} to discuss representations of the quiver indicated in Fig.~\ref{fig:quiver1} in the following example.



%%
%%---------------------------------------Example---------------------------------------------------------------------
%%

\begin{example}\normalfont
Taking into account the quiver discussed in example~\ref{example:1}, we can have the following representation: The vector spaces associated to the nodes are $\mathcal{V}_{1}=\mathbb{R}^{2}$, $\mathcal{V}_{2}=\mathbb{R}^{2,2}$, $\mathcal{V}_{3}=\mathbb{R}^{5,5}$, $\mathcal{V}_{4}=\mathbb{R}^{3}$, $\mathcal{V}_{5}=\mathbb{R}$ while the linear maps are given by
%
%
\begin{equation*}
\phi_{1,2}(\mathbf{x})=\mathbf{1}_{1\times2}\otimes\mathbf{x},\quad\phi_{1,3}(\mathbf{x})=\mathbf{1}_{1\times 5}\otimes\mathbf{x},\quad\phi_{2,2}(\mathbf{x})=3\bbx
\end{equation*}
%
%
\begin{equation*}
\phi_{2,3}(\bbx)=
\begin{pmatrix} 
\mathbf{x}                     & \mathbf{0}_{2\times 3}\\
\mathbf{0}_{3\times 2} &  \mathbf{0}_{3\times 3}
\end{pmatrix}
,\quad
\phi_{3,4}(\bbx)=[\bbx]_{(1:3),(1:3)},
\end{equation*}
%
%
\begin{equation*}
\quad \phi_{4,4}(\bbx)=\bbI_{4\times 4}\bbx,\quad \phi_{4,1}(\bbx)=[\bbx(1)+\bbx(2),\bbx(2)+\bbx(3)]^{T}
\end{equation*}
%
%
\begin{equation*}
\phi_{3,5}(\bbx)=\mathbf{1}_{1\times 5}\bbx\mathbf{1}_{5\times 1},\quad\phi_{5,1}(\bbx)=[\bbx,\bbx]^{T}
\end{equation*}
%
%
where $\mathbb{R}^{k,k}$ indicates the set of matrices of size $k\times k$ with entries in $\mathbb{R}$, $\mathbb{R}^{k}$ is the $k-$dimensional Euclidean space, $\mathbf{1}_{r\times k}$ and $\mathbf{0}_{r\times k}$ are the all ones array and the all zeros array of dimensions $r\times k$ while $\times$ denotes the Kronecker product. The symbol $[\bbx]_{(1:r),(1:k)}$ represents the array obtained keeping the first $r$ rows and the first $k$ columns of $\bbx$. 
\end{example}

%%
%%---------------------------------------End of Example---------------------------------------------------------------------
%%


%%
%%---------------------------------------Example---------------------------------------------------------------------
%%

\begin{example}\normalfont
\blue{Dear Hans: Here we can add an example of a quiver that arises naturally from an example in computational topology or anything related}
\end{example}

%%----------------------------------End of Example----------------------------------------------------------------


The notion of quiver representations  is naturally embeded in the context of the representation theory of algebras~\cite{repthysmbook,derksen2017introduction,kirillov2016quiver}. Therefore, it is possible to talk about irreducible representations, indecomposable representations and so on. In what follows we proceed to introduce these notions for quivers, which will be later used to define a signal processing framework. 

We start with a notion that will allow us to compare representations of a quiver.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% DEFINITION %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{definition}
Let $\boldsymbol{\pi}_{1}$ and $\boldsymbol{\pi}_{2}$ be two representations of a quiver $Q=(Q_{0},Q_{1},h,t)$. We get a morphism $\phi:\boldsymbol{\pi}_{1}\rightarrow\boldsymbol{\pi}_{2}$ if we attach to every vertex $x\in Q_{0}$ a $\mathbb{C}-$linear map $\phi(x):\boldsymbol{\pi}_{1}(x)\rightarrow\boldsymbol{\pi}_{2}(x)$ such that for every $a\in Q_{1}$ the following diagram commutes
%
\begin{center}
\begin{tikzcd}
\boldsymbol{\pi}_{1}(t(a)) \arrow[r, "\boldsymbol{\pi}_{1}(a)"] \arrow[d, "\phi(t(a))"]
& \boldsymbol{\pi}_{1}(h(a)) \arrow[d, "\phi(h(a))" ] \\
\boldsymbol{\pi}_{2}(t(a)) \arrow[r, "\boldsymbol{\pi}_{2}(a)" ]
& \boldsymbol{\pi}_{2}(h(a)) 
\end{tikzcd}
\end{center}
%
i.e. $\phi(h(a))\boldsymbol{\pi}_{1}(a)=\boldsymbol{\pi}_{2}(a)\phi(t(a))$. We say that $\phi$ is an isomorphism if $\phi(x)$ is invertible for all $x$.
\end{definition}

%%%%%%%%%%End of DEFINITION %%%%%%%%%%%

For any two representations $\boldsymbol{\pi}_{1}$ and $\boldsymbol{\pi}_{2}$ of a quiver $Q$, their direct sum is given according to $(\boldsymbol{\pi}_{1}\oplus\boldsymbol{\pi}_{2})(x)=\boldsymbol{\pi}_{1}(x)\oplus\boldsymbol{\pi}_{2}(x)$ whether $x$ is in $Q_{0}$ or $Q_{1}$~\cite{derksen2017introduction}. Additionally, we will call a representation $\boldsymbol{\pi}$ trivial if $\boldsymbol{\pi}(x)=\mathbf{0}$ for all $x\in Q_{0}$.

Now, we are ready to introduce the notion of decomposable (indecomposable) and irreducible representation. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% DEFINITION %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{definition}
A nontrivial representation $\boldsymbol{\pi}$ of a quiver $Q$ is called decomposable if $\boldsymbol{\pi}$ is isomorphic to $(\boldsymbol{\pi}_{1}\oplus\boldsymbol{\pi}_{2})$ for some nontrivial representations 
$\boldsymbol{\pi}_{1}, \boldsymbol{\pi}_{2}$ of $Q$. A nontrivial representation that is not decomposable is called indecomposable. A nontrivial representation $\boldsymbol{\pi}$ is called irreducible or simple if for every subrepresentation $\boldsymbol{\theta}$ of $\boldsymbol{\pi}$, $\boldsymbol{\theta}$ is trivial or equal to $\boldsymbol{\pi}$.
\end{definition}

%%%%%%%%%%End of DEFINITION %%%%%%%%%%%

It is important to point out that this notion of representation is connected indeed connected with the traditional notions of decomposability and irreducibility for associative algebras~\cite{derksen2017introduction,repthysmbook} considering the so called \textit{path algebra}. A path $p$ in a quiver $Q=(Q_{0},Q_{1},h,t)$ of length $\ell\geq 1$ is a sequence $q=a_{\ell}a_{\ell-1}\ldots a_{1}$ of arrows in $Q_{1}$ such that $t(a_{i+1})=h(a_{i})$ for $i=1,\ldots,\ell-1$ with $h(p)=h(a_{\ell})$ and $t(p)=t(a_{1})$~\cite{derksen2017introduction}. In this context a trivial path $e_{x}$ of length zero can be defined by $h(e_{x})=t(e_{x})=x$. If $\boldsymbol{\pi}$ is a representation of Q, we can the define $\boldsymbol{\pi}(p)=\boldsymbol{\pi}(a_{\ell})\boldsymbol{\pi}(a_{\ell-1})\cdots \boldsymbol{\pi}(a_{1})$ and for $x\in Q_{0}$ we can define $\boldsymbol{\pi}(e_{x}):=1_{\boldsymbol{\pi}(x)}:\boldsymbol{\pi}(x)\rightarrow\boldsymbol{\pi}(x)$. Notice that for any paths $p,q$ we have that $\boldsymbol{\pi}(p)\boldsymbol{\pi}(q)=\boldsymbol{\pi}(pq)$ whenever $t(p)=h(q)$~\cite{derksen2017introduction,repthysmbook}.

\blue{---AlejandroPM: I am working here, I will improve this portion later----
The path algebra $\mathcal{A_{P}}$ is the $\mathbb{C}-$algebra with basis given by all the paths in $Q$. If we take any two elements $\vec{p},\vec{q}$ in $\mathcal{A_{P}}$, i.e. two paths $p,q$ in $Q$ we can define a product in $\mathcal{A_{P}}$ given by
%
\begin{equation}
\vec{p}\vec{q}=\left\lbrace
\begin{matrix}
\overrightarrow{pq}  & \text{if} & t(p)=h(q)\\
\vec{0}    & \text{if} &  t(p)\neq h(q)
\end{matrix}
\right.
\end{equation}
%
notice that $pq$ indicates the concatenation of paths.-----}

Relying on the associative algebra $\mathcal{A_{P}}$ we can formally define a signal processing framework in the sense of~\cite{algSP0,algSP1,algSP2,algSP3}, introduce then the notions of Fourier decompositions and unleash a complete theory of signal processing. Before we proceed to do so, we take into account that as pointed out in~\cite{derksen2017introduction} (page 12, proposition 1.5.4), the category\footnote{Here and after we use the word \textit{category} in the context of category theory.} of representations of a quiver is equivalent to the category of representations of its path algebra, this means that in terms of determining representations and its properties we can work either with the quiver directly or with its path algebra. However, As dicussed in~\cite{repthysmbook} (page 20, remark 2.8.7) in general it is easier to work with the representations of the quiver directly without using the path algebra.

Then, we proceed to develop the notion of signal processing on quivers under the umbrella of algebraic signal processing as stated in~\cite{algSP0,algSP1,algSP2,algSP3}, but working directly with the quiver representation. As we will show, we can define the notions of Fourier decomposition and filtering.














==> sec_spquiverep.tex <==
%!TEX root = quiverSP_v00.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% INTRODUCTION %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Signal Processing on Quiver Representations}
\label{sec:spquiverep}

We start with introducing the notion of \textit{signal} on the representation of a quiver as follows.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% DEFINITION %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{definition}\label{def:quiversig}
Let $Q=(Q_{0},Q_{1},h,t)$ a quiver and $\boldsymbol{\pi}$ a representation of $Q$. Then a signal $\mathbf{x}$ on $\boldsymbol{\pi}$ is defined according to the map
%
\begin{equation}
\mathbf{x}: Q_{0}\rightarrow\boldsymbol{\pi}(Q_{0}).
\end{equation}
%
\end{definition}

%%%%%% END DEFINITION %%%%%%%%%%%%%%

For the sake of clarity, in what follows we denote by the triple $(Q,\boldsymbol{\pi},\bbx)$ a quiver signal on the quiver $Q$ taking its values on the representation $\boldsymbol{\pi}$.

To illustrate what a signal on a quiver looks like let us consider the following example. 


%%--------------------------------------------------------------------
%%----------------------Example----------------------------------
%%--------------------------------------------------------------------

\begin{example}
Let us recall the examples and 1 and 2, where we discuss the quiver $Q$ illustrated in Fig.~\ref{xx}. An example of a signal $\bbx$ on $Q$ taking values in the representation $\boldsymbol{\pi}$ illustrated in example 2 is given by 
%
%
\begin{equation*}
\bbx(1)=[1,1]^{T},\quad \bbx(2)=2\bbI_{2\times 2},\quad\bbx(3)=5\bbI_{5\times 5}
\end{equation*}
%
%
\begin{equation*}
\bbx(4)=[1,0,1]^{T},\quad \bbx(5)=8
\end{equation*}
%
%
\end{example}

%%------------------End of Example---------------------------

Then a signal defined on the representation of a quiver assigns quantities of different \textit{nature} and dimension to every node of the quiver.


==> source_figs/figs_gnn/atNode.tex <==
%!TEX root = ../gnn_swarm_intel.tex

\def \thisplotscale {0.4}
\def \unit {\thisplotscale cm}

\tikzstyle {block} = [draw,
                      rectangle, 
                      fill = blue!10, 
                      minimum height = 2*\unit]

\tikzstyle {long block}  = [block,
                            minimum width = 4*\unit]

\tikzstyle {short block} = [block,
                            minimum width = 2*\unit]

\tikzstyle {circle block}   = [draw,
                            circle,
                            minimum width = 0.9*\unit]

\def\blockDistance{7}


{\footnotesize\begin{tikzpicture}[x = 1*\unit, y=1*\unit, font=\footnotesize]

% Origin
\node at (0,0) (O) {};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Draw all blocks
%
% Block for aggregator
\path(O) node (zn) {\includegraphics[width=0.2300\textwidth]{figs_gnn/AggregationCNNGSLayer1Input.pdf}};
% Block for CNN
\path (zn.east) ++ (\blockDistance,0) node [long block] (CNN) {CNN};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Draw all arrows
%
% Arrow into CNN
\path [draw, -stealth] (zn.east) -- (CNN.west)  node  [midway, above] (z) {$\bbz_{in}$};
% Arrow out of CNN
\path [draw, -stealth] (CNN.east) -++ (0.5*\blockDistance,0)  node  [midway,above] (outCNN) {$\bbu_{in}$};


\end{tikzpicture}}




==> source_figs/figs_gnn/cnn_block_diagram_single_feature.tex <==
% !TEX root = ../00_gnn_eusipco.tex

\def \myfactor {0.65}
\def \unit  {\myfactor cm}

% Definition of a block for block diagrams
\tikzstyle{block} = [ rectangle,
                      minimum width = \unit,
                      minimum height = \unit,
                      fill = blue!15,
                      draw = black,
                      text = black]

% Control the color and size of filter blocks                  
\tikzstyle{filter} = [ block,
                      minimum width  = 4.0*\unit,
                      minimum height = 1.3*\unit]

% Control the color and size of nonlinearity blocks 
\tikzstyle{nonlinearity} = [ filter,
                             minimum width  = 4.0*\unit,
                             fill = mygreen!15]

% Control separation between blocks
\def \deltainput     {( 0.0,-1.5)}
\def \deltaoutput    {( 0.0,-0.9)}
\def \deltalayer     {3.0}
\def \deltaconnector {0.95}
\def \deltasigma     {( 5.0, 0.0)}
\def \deltafeature   {1.5}

% The text that is displayed inside of filter blocks
\def \one   {$\displaystyle{\bbz_1  = \sum_{k=0}^\infty \red{h_{1k}}\bbS^k\, \bbx    }$}
\def \two   {$\displaystyle{\bbz_1  = \sum_{k=0}^\infty \red{h_{2k}}\bbS^k\, \bbx_{1}}$}
\def \three {$\displaystyle{\bbz_1  = \sum_{k=0}^\infty \red{h_{3k}}\bbS^k\, \bbx_{2}}$}
% The text that is displayed inside of nonlinearity blocks
\def \sigmaone   {$\displaystyle{\bbx_{1} = \red{\sigma} \Big[\, \bbz_1 \, \Big]}$}
\def \sigmatwo   {$\displaystyle{\bbx_{2} = \red{\sigma} \Big[\, \bbz_2 \, \Big]}$}
\def \sigmathree {$\displaystyle{\bbx_{3} = \red{\sigma} \Big[\, \bbz_3 \, \Big]}$}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BEGIN FIGURE CODE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
{\fontsize{7}{7}\selectfont\begin{tikzpicture}[scale = \myfactor]

  \pgfdeclarelayer{bg}     % declare background layer
  \pgfsetlayers{bg,main}   % set the order of the layers (main is the standard layer)

  % Draw input to GNN
  \node (input) [rectangle, minimum width = 0.1*\unit] {$\bbx$};
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Layer 1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Draw Layer 1 Filter block and Feature block
  \path (input)      ++ \deltainput node [filter]       (L1 Filter1) {\one};
  \path (L1 Filter1) ++ \deltasigma node [nonlinearity] (L1 F1)      {\sigmaone};
  % Draw connectors for Layer 1
  \path[draw, -stealth] (L1 Filter1.east) -- node [above] {$\bbz_1$} (L1 F1.west);

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Layer 2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Draw Layer 2 Filter block and Feature block
  \path (L1 Filter1) ++ (0,-\deltalayer) node [filter]       (L2 Filter1) {\two};
  \path (L2 Filter1) ++ \deltasigma      node [nonlinearity] (L2 F1)      {\sigmatwo};
  % Draw connectors for Layer 2
  \path[draw, -stealth] (L2 Filter1.east) --  node [above] {$\bbz_2$} (L2 F1.west);
  
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Layer 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Draw Layer 2 Filter block and Feature block
  \path (L2 Filter1) ++ (0,-\deltalayer) node [filter]       (L3 Filter1) {\three};
  \path (L3 Filter1) ++ \deltasigma      node [nonlinearity] (L3 F1)      {\sigmathree};
  % Draw connectors for Layer 2
  \path[draw, -stealth] (L3 Filter1.east) --  node [above] {$\bbz_3$} (L3 F1.west);

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Connections across layers %%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % From input to layer 1
  \path[draw, -stealth] (input.south) -- (L1 Filter1.north);
  % From layer 1 to layer 2
  \path (L1 F1.south) ++ (0,-\deltaconnector) node [] (aux1) {};
  \path[draw, -stealth] (L1 F1.south) -- node [below right] {$\bbx_1$} (aux1.north) 
                                      --                         (aux1.north -| L2 Filter1.north) 
                                      -- node [above left]  {$\bbx_1$} (L2 Filter1.north);
  % From layer 2 to layer 3
  \path (L2 F1.south) ++ (0,-\deltaconnector) node [] (aux1) {};
  \path[draw, -stealth] (L2 F1.south) -- node [below right] {$\bbx_2$} (aux1.north) 
                                      --                         (aux1.north -| L2 Filter1.north) 
                                      -- node [above left]  {$\bbx_2$} (L3 Filter1.north);
  % From layer 3 to output
  \path[draw, -stealth] (L3 F1.south) -- ++ \deltaoutput -- ++ (0.3, 0) 
                        node [right]{\red{$\bbx_3 = \bbPhi(\bbx; \bbH)$}};

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Light shades to signify layer groups   %%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{pgfonlayer}{bg} 
      % Shading for Layer 1  
      \path (L1 Filter1.west |- L1 F1.south) ++ (-0.3,-0.3)
           node [filter, anchor = south west,
                 fill = black!1, 
                 minimum width  = 10.75*\unit,
                 minimum height = 1.9*\unit,] 
        (layer)
        {}; 
      \path (layer.south east) ++ (0.0,0.0) node [above left] {\fontsize{6}{6}\selectfont Layer 1};
      % Shading for Layer 2  
      \path (L1 Filter1.west |- L2 F1.south) ++ (-0.3,-0.3)
           node [filter, anchor = south west,
                 fill = black!1, 
                 minimum width  = 10.75*\unit,
                 minimum height = 1.9*\unit,] 
        (layer)
        {}; 
      \path (layer.south east) ++ (0.0,0.0) node [above left] {\fontsize{6}{6}\selectfont Layer 2};
      % Shading for Layer 3  
      \path (L1 Filter1.west |- L3 F1.south) ++ (-0.3,-0.3)
           node [filter, anchor = south west,
                 fill = black!1, 
                 minimum width  = 10.75*\unit,
                 minimum height = 1.9*\unit,] 
        (layer)
        {}; 
      \path (layer.south east) ++ (0.0,0.0) node [above left] {\fontsize{6}{6}\selectfont Layer 3};

  \end{pgfonlayer}


\end{tikzpicture}} 


==> source_figs/figs_gnn/gnn_block_diagram_single_feature.tex <==
% !TEX root = ../00_gnn_eusipco.tex

\def \myfactor {0.65}
\def \unit  {\myfactor cm}

% Definition of a block for block diagrams
\tikzstyle{block} = [ rectangle,
                      minimum width = \unit,
                      minimum height = \unit,
                      fill = blue!15,
                      draw = black,
                      text = black]

% Control the color and size of filter blocks                  
\tikzstyle{filter} = [ block,
                      minimum width  = 4.0*\unit,
                      minimum height = 1.3*\unit]

% Control the color and size of nonlinearity blocks 
\tikzstyle{nonlinearity} = [ filter,
                             minimum width  = 4.0*\unit,
                             fill = mygreen!15]

% Control separation between blocks
\def \deltainput     {( 0.0,-1.5)}
\def \deltaoutput    {( 0.0,-0.9)}
\def \deltalayer     {3.0}
\def \deltaconnector {0.95}
\def \deltasigma     {( 5.0, 0.0)}
\def \deltafeature   {1.5}

% The text that is displayed inside of filter blocks
\def \one   {$\displaystyle{\bbz_1  = \sum_{k=0}^\infty {h_{1k}}\red{\bbS^k}\, \bbx    }$}
\def \two   {$\displaystyle{\bbz_1  = \sum_{k=0}^\infty {h_{2k}}\red{\bbS^k}\, \bbx_{1}}$}
\def \three {$\displaystyle{\bbz_1  = \sum_{k=0}^\infty {h_{3k}}\red{\bbS^k}\, \bbx_{2}}$}
% The text that is displayed inside of nonlinearity blocks
\def \sigmaone   {$\displaystyle{\bbx_{1} = {\sigma} \Big[\, \bbz_1 \, \Big]}$}
\def \sigmatwo   {$\displaystyle{\bbx_{2} = {\sigma} \Big[\, \bbz_2 \, \Big]}$}
\def \sigmathree {$\displaystyle{\bbx_{3} = {\sigma} \Big[\, \bbz_3 \, \Big]}$}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BEGIN FIGURE CODE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
{\fontsize{7}{7}\selectfont\begin{tikzpicture}[scale = \myfactor]

  \pgfdeclarelayer{bg}     % declare background layer
  \pgfsetlayers{bg,main}   % set the order of the layers (main is the standard layer)

  % Draw input to GNN
  \node (input) [rectangle, minimum width = 0.1*\unit] {$\bbx$};
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Layer 1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Draw Layer 1 Filter block and Feature block
  \path (input)      ++ \deltainput node [filter]       (L1 Filter1) {\one};
  \path (L1 Filter1) ++ \deltasigma node [nonlinearity] (L1 F1)      {\sigmaone};
  % Draw connectors for Layer 1
  \path[draw, -stealth] (L1 Filter1.east) -- node [above] {$\bbz_1$} (L1 F1.west);

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Layer 2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Draw Layer 2 Filter block and Feature block
  \path (L1 Filter1) ++ (0,-\deltalayer) node [filter]       (L2 Filter1) {\two};
  \path (L2 Filter1) ++ \deltasigma      node [nonlinearity] (L2 F1)      {\sigmatwo};
  % Draw connectors for Layer 2
  \path[draw, -stealth] (L2 Filter1.east) --  node [above] {$\bbz_2$} (L2 F1.west);
  
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Layer 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Draw Layer 2 Filter block and Feature block
  \path (L2 Filter1) ++ (0,-\deltalayer) node [filter]       (L3 Filter1) {\three};
  \path (L3 Filter1) ++ \deltasigma      node [nonlinearity] (L3 F1)      {\sigmathree};
  % Draw connectors for Layer 2
  \path[draw, -stealth] (L3 Filter1.east) --  node [above] {$\bbz_3$} (L3 F1.west);

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Connections across layers %%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % From input to layer 1
  \path[draw, -stealth] (input.south) -- (L1 Filter1.north);
  % From layer 1 to layer 2
  \path (L1 F1.south) ++ (0,-\deltaconnector) node [] (aux1) {};
  \path[draw, -stealth] (L1 F1.south) -- node [below right] {$\bbx_1$} (aux1.north) 
                                      --                         (aux1.north -| L2 Filter1.north) 
                                      -- node [above left]  {$\bbx_1$} (L2 Filter1.north);
  % From layer 2 to layer 3
  \path (L2 F1.south) ++ (0,-\deltaconnector) node [] (aux1) {};
  \path[draw, -stealth] (L2 F1.south) -- node [below right] {$\bbx_2$} (aux1.north) 
                                      --                         (aux1.north -| L2 Filter1.north) 
                                      -- node [above left]  {$\bbx_2$} (L3 Filter1.north);
  % From layer 3 to output
  \path[draw, -stealth] (L3 F1.south) -- ++ \deltaoutput -- ++ (0.3, 0) 
                        node [right]{$\bbx_3 = \bbPhi(\bbx; \bbH, \red{\bbS})$};

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Light shades to signify layer groups   %%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{pgfonlayer}{bg} 
      % Shading for Layer 1  
      \path (L1 Filter1.west |- L1 F1.south) ++ (-0.3,-0.3)
           node [filter, anchor = south west,
                 fill = black!1, 
                 minimum width  = 10.75*\unit,
                 minimum height = 1.9*\unit,] 
        (layer)
        {}; 
      \path (layer.south east) ++ (0.0,0.0) node [above left] {\fontsize{6}{6}\selectfont Layer 1};
      % Shading for Layer 2  
      \path (L1 Filter1.west |- L2 F1.south) ++ (-0.3,-0.3)
           node [filter, anchor = south west,
                 fill = black!1, 
                 minimum width  = 10.75*\unit,
                 minimum height = 1.9*\unit,] 
        (layer)
        {}; 
      \path (layer.south east) ++ (0.0,0.0) node [above left] {\fontsize{6}{6}\selectfont Layer 2};
      % Shading for Layer 3  
      \path (L1 Filter1.west |- L3 F1.south) ++ (-0.3,-0.3)
           node [filter, anchor = south west,
                 fill = black!1, 
                 minimum width  = 10.75*\unit,
                 minimum height = 1.9*\unit,] 
        (layer)
        {}; 
      \path (layer.south east) ++ (0.0,0.0) node [above left] {\fontsize{6}{6}\selectfont Layer 3};

  \end{pgfonlayer}


\end{tikzpicture}} 


==> source_figs/figs_gnn/gnn_block_diagram_single_feature_uncolored.tex <==
% !TEX root = ../00_gnn_eusipco.tex

\def \myfactor {0.65}
\def \unit  {\myfactor cm}

% Definition of a block for block diagrams
\tikzstyle{block} = [ rectangle,
                      minimum width = \unit,
                      minimum height = \unit,
                      fill = blue!15,
                      draw = black,
                      text = black]

% Control the color and size of filter blocks                  
\tikzstyle{filter} = [block,
                      minimum width  = 4.0*\unit,
                      minimum height = 1.3*\unit,
                      fill=blue!15!cyan!80!white]

% Control the color and size of nonlinearity blocks 
\tikzstyle{nonlinearity} = [ filter,
                             minimum width  = 4.0*\unit,
                             fill = gray!30!white]
                             %fill = mygreen!15]

% Control separation between blocks
\def \deltainput     {( 0.0,-1.5)}
\def \deltaoutput    {( 0.0,-0.9)}
\def \deltalayer     {3.0}
\def \deltaconnector {0.95}
\def \deltasigma     {( 5.0, 0.0)}
\def \deltafeature   {1.5}

% The text that is displayed inside of filter blocks
\def \one   {$\displaystyle{\boldsymbol{z}_{1}  = \rho_{1}(a)\boldsymbol{x}}$}
\def \two   {$\displaystyle{\boldsymbol{z}_2  =  \rho_{2}(a)\boldsymbol{x}_{1}}$}
\def \three {$\displaystyle{\boldsymbol{z}_3  = \rho_{3}(a)\boldsymbol{x}_{2}}$}
% The text that is displayed inside of nonlinearity blocks
\def \sigmaone   {$\displaystyle{\boldsymbol{x}_{1} = {\sigma} \Big[\, \boldsymbol{z}_1 \, \Big]}$}
\def \sigmatwo   {$\displaystyle{\boldsymbol{x}_{2} = {\sigma} \Big[\, \boldsymbol{z}_2 \, \Big]}$}
\def \sigmathree {$\displaystyle{\boldsymbol{x}_{3} = {\sigma} \Big[\, \boldsymbol{z}_3 \, \Big]}$}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BEGIN FIGURE CODE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
{\fontsize{7}{7}\selectfont\begin{tikzpicture}[scale = \myfactor]

  \pgfdeclarelayer{bg}     % declare background layer
  \pgfsetlayers{bg,main}   % set the order of the layers (main is the standard layer)

  % Draw input to GNN
  \node (input) [rectangle, minimum width = 0.1*\unit] {$\boldsymbol{x}$};
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Layer 1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Draw Layer 1 Filter block and Feature block
  \path (input)      ++ \deltainput node [filter]       (L1 Filter1) {\one};
  \path (L1 Filter1) ++ \deltasigma node [nonlinearity] (L1 F1)      {\sigmaone};
  % Draw connectors for Layer 1
  \path[draw, -stealth] (L1 Filter1.east) -- node [above] {$\boldsymbol{z}_1$} (L1 F1.west);

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Layer 2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Draw Layer 2 Filter block and Feature block
  \path (L1 Filter1) ++ (0,-\deltalayer) node [filter]       (L2 Filter1) {\two};
  \path (L2 Filter1) ++ \deltasigma      node [nonlinearity] (L2 F1)      {\sigmatwo};
  % Draw connectors for Layer 2
  \path[draw, -stealth] (L2 Filter1.east) --  node [above] {$\boldsymbol{z}_2$} (L2 F1.west);
  
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Layer 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Draw Layer 2 Filter block and Feature block
  \path (L2 Filter1) ++ (0,-\deltalayer) node [filter]       (L3 Filter1) {\three};
  \path (L3 Filter1) ++ \deltasigma      node [nonlinearity] (L3 F1)      {\sigmathree};
  % Draw connectors for Layer 2
  \path[draw, -stealth] (L3 Filter1.east) --  node [above] {$\boldsymbol{z}_3$} (L3 F1.west);

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Connections across layers %%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % From input to layer 1
  \path[draw, -stealth] (input.south) -- (L1 Filter1.north);
  % From layer 1 to layer 2
  \path (L1 F1.south) ++ (0,-\deltaconnector) node [] (aux1) {};
  \path[draw, -stealth] (L1 F1.south) -- node [below right] {$\boldsymbol{x}_1$} (aux1.north) 
                                      --                         (aux1.north -| L2 Filter1.north) 
                                      -- node [above left]  {$\boldsymbol{x}_1$} (L2 Filter1.north);
  % From layer 2 to layer 3
  \path (L2 F1.south) ++ (0,-\deltaconnector) node [] (aux1) {};
  \path[draw, -stealth] (L2 F1.south) -- node [below right] {$\boldsymbol{x}_2$} (aux1.north) 
                                      --                         (aux1.north -| L2 Filter1.north) 
                                      -- node [above left]  {$\boldsymbol{x}_2$} (L3 Filter1.north);
  % From layer 3 to output
  \path[draw, -stealth] (L3 F1.south) -- ++ \deltaoutput -- ++ (0.3, 0) 
                        node [right]{$\boldsymbol{x}_3 = \red{\bbPhi_{\Xi}\boldsymbol{x}}$};

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Light shades to signify layer groups   %%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{pgfonlayer}{bg} 
      % Shading for Layer 1  
      \path (L1 Filter1.west |- L1 F1.south) ++ (-0.3,-0.3)
           node [filter, anchor = south west,
                 fill = black!1, 
                 %minimum width  = 10.75*\unit,
                 minimum width  = 12*\unit,
                 minimum height = 1.9*\unit,] 
        (layer)
        {}; 
      %\path (layer.south east) ++ (0.0,0.0) node [above left] {\fontsize{6}{6}\selectfont Layer 1};
       \path (layer.south east) ++ (0.0,0.0) node [above left] {\fontsize{6}{6}\selectfont  $\boldsymbol{x}_{1}\in\mathcal{M}_{2}$};
 \path (layer.south east) ++ (0.0,1) node [above left] {\fontsize{6}{6}\selectfont  $a\in\mathcal{A}_{1}$};
  \path (layer.south east) ++ (0.0,0.5) node [above left] {\fontsize{6}{6}\selectfont  $\boldsymbol{z}_{1}\in\mathcal{M}_{1}$};
      % Shading for Layer 2  
      \path (L1 Filter1.west |- L2 F1.south) ++ (-0.3,-0.3)
           node [filter, anchor = south west,
                 fill = black!1, 
                 minimum width  = 12*\unit,
                 minimum height = 1.9*\unit,] 
        (layer)
        {}; 
      %\path (layer.south east) ++ (0.0,0.0) node [above left] {\fontsize{6}{6}\selectfont Layer 2};
      \path (layer.south east) ++ (0.0,0.0) node [above left] {\fontsize{6}{6}\selectfont  $\boldsymbol{x}_{2}\in\mathcal{M}_{3}$};
 \path (layer.south east) ++ (0.0,1) node [above left] {\fontsize{6}{6}\selectfont  $a\in\mathcal{A}_{2}$};
  \path (layer.south east) ++ (0.0,0.5) node [above left] {\fontsize{6}{6}\selectfont  $\boldsymbol{z}_{2}\in\mathcal{M}_{2}$};
      % Shading for Layer 3  
      \path (L1 Filter1.west |- L3 F1.south) ++ (-0.3,-0.3)
           node [filter, anchor = south west,
                 fill = black!1, 
                 minimum width  = 12*\unit,
                 minimum height = 1.9*\unit,] 
        (layer)
        {}; 
      \path (layer.south east) ++ (0.0,0.0) node [above left] {\fontsize{6}{6}\selectfont  $\boldsymbol{x}_{3}\in\mathcal{M}_{\text{out}}$};
 \path (layer.south east) ++ (0.0,1) node [above left] {\fontsize{6}{6}\selectfont  $a\in\mathcal{A}_{3}$};
  \path (layer.south east) ++ (0.0,0.5) node [above left] {\fontsize{6}{6}\selectfont  $\boldsymbol{z}_{3}\in\mathcal{M}_{3}$};
  \end{pgfonlayer}

\end{tikzpicture}} 

